HPP: Hierarchical Programmatic Probing for Long Video Understanding by Decoupling Perception and Reasoning

Understanding long videos requires fine-grained perception and multi-step, higher-order reasoning over complex, long-range spatio-temporal dynamics. Vision-language models (VLMs) encode video frames into visual tokens and attempt to perform both perception and multi-step planning latently, within a single forward pass. This coupled formulation, however, is bottlenecked by the LLM's limited capacity to discover and execute multi-step strategies in its latent representations. To address this bottleneck, we propose Hierarchical Programmatic Probing (HPP), a framework that decouples semantic perception from higher-order temporal reasoning by reformulating long video understanding as iterative, programmatic exploration of a hierarchically segmented video. Specifically, a coding-capable LLM plans and executes a multi-step strategy in an interactive coding environment, probing the video for information and invoking a VLM for localized perception on demand. To make probing tractable over long videos, we introduce three components: information-density-aware hierarchical segmentation, late-interaction semantic retrieval, and structured probing functions for coarse-to-fine temporal localization. We validate HPP on LongVideoBench, which requires both fine-grained perception and long-range relational reasoning, and show that decoupling the two via iterative programmatic probing yields substantial gains. Further results on EgoSchema, VideoMME, and MLVU demonstrate the effectiveness of our approach across diverse long-video benchmarks.

==> search_v1.tex <==

After dividing a video into manageable segments, the next step is to enable the LLM to retrieve query-relevant content via text. Video retrieval methods typically employ a bi-encoder architecture, in which frames are uniformly sampled from a video segment, encoded using a vision encoder, and aggregated into a single global embedding~\cite{shu2024videoxl, xu2021videoclip}. This global representation, together with a text embedding, is then used to compute similarity and retrieve relevant results.

However, unlike general video retrieval, text-based localization within a single video requires a more fine-grained approach, as different segments may share substantial visual similarity. For example, localizing a segment corresponding to the query “bird flying over water” in a nature documentary requires distinguishing it from visually similar scenes of birds flying over a desert. Moreover, motion dynamics can vary significantly across short segments, making uniform frame sampling suboptimal. To address these challenges, we design a video localization method that adaptively samples frames based on the magnitude of motion within each shot and computes similarity using late interaction between independently encoded shot and query embeddings~\cite{khattab2020colbert, reddy2025video}.


The localization is performed at the segment level (e.g., shots). Let $\{s_i\}_{i=1}^{N}$ denote the set of shots for a video, where each shot $s_i$ contains $T_{s_i}$ frames $\{f_{i, t}\}_{t=1}^{T_{s_i}}$ and a keyframe. We sample frames proportionally to the shot's motion energy $\gamma_i$ computed using Eq.~\ref{eq:gamma}. The number of sampled frames for the $i$-th shot is given by
$$\eta_i = \frac{\gamma_i}{\sum_{m=1}^{N} \gamma_m} \, B_{\text{total}},$$
where $B_{\text{total}}$ is total frame budget.  
% 
% 
For each shot $s_i$, $\eta_i$ frames $\{f_{i,k}\}_{k=1}^{\eta_i}$ are sampled and encoded using a CLIP-like vision encoder $\phi_v$ to obtain frame-level embeddings
$
\mathbf{z}_{i, t} = \phi_v(f_{i,t}) \in \mathbb{R}^{d}.
$
Similarly, a textual query consisting of $n_t$ tokens ${q_l}_{l=1}^{n_t}$ is encoded using a text encoder $\phi_t$ to obtain token-level embeddings
$
\mathbf{q_l} = \phi_t(q_l) \in \mathbb{R}^{d}.
$


To capture fine-grained token–frame interactions within each shot while maintaining the efficiency of dot-product similarity, we compute a weighted late-interaction MaxSim score
\[
\text{MaxSim}(q, s_j) 
= 
\frac{1}{\eta_i} 
\sum_{k=1}^{\eta_i} 
w_{j,k} \cdot 
\max_{i} 
\left( 
\mathbf{q}_i^\top \mathbf{z}_{j,k} 
\right),
\]
where $w_{j,k}$ is the weight of the $k$-th frame in shot $s_i$, assigning higher importance to keyframes. This per-token motion-adaptive per-frame interaction captures fine-grained and dynamic spatio-temporal information.  
% 
To further capture shot-level global information, we aggregate frame and query embeddings via mean pooling:
$
\mathbf{z}_i 
= 
\frac{1}{\eta_i} 
\sum_{t=1}^{\eta_i} 
\mathbf{z}_{j,t},
$
and $
\mathbf{q} 
= 
\frac{1}{n_t} 
\sum_{i=1}^{n_t} 
\mathbf{q}_i,
$
and compute a shot-level similarity with the query:
$
\text{Sim}(q, s_j) 
= 
\mathbf{q}^\top \mathbf{z}_i.
$
% 
The final similarity score combines fine-grained and global similarities:
$
\text{score}(q, s_j) 
= \alpha_s \cdot \text{MaxSim}(q, s_j)+ (1-\alpha_s) \cdot \text{Sim}(q, s_j),
$
where $\alpha_s$ is a weighting hyperparameter. 
% 
By modeling both global shot-level semantics and fine-grained token–frame interactions, the search module captures static spatial context as well as motion-driven action cues, leading to more precise and reliable localization.
% 
Top-$k$ candidate shots are returned along with their similarity scores, which LLM can use to decide which shots to further probe.  
% 
Scenes are not embedded separately; instead, a scene representation is computed by using the embeddings of its constituent shots, reducing computation while preserving semantic structure.

 \begin{table}[t]                                                                                                                
  \centering
  \caption{VLM accuracy (\%) on LongVideoBench.}
  \label{tab:vlm_results}         
  \setlength{\tabcolsep}{3pt}
  \footnotesize                   
  \begin{tabular}{l l l cc cc c}    \toprule                             
  & & & \multicolumn{2}{c}{\textbf{LVB3600}} & \multicolumn{2}{c}{\textbf{Avg}} & \\
  \cmidrule(lr){4-5} \cmidrule(lr){6-7}                           
  \textbf{LLM} & \textbf{VLM} & \textbf{V.E.} & L1 & L2 & L1 & L2 & \textbf{All} \\                                           
  \midrule                         
  Kimi-K2  & 2B& 0.3B   & 68.0 & 60.0 & 69.1 & 67.6 & 68.3 \\                                                
  % Gemma-3-4B      & SigLIP       & Gemma3-4B  & 45.1 & 27.3 & 55.3 & 44.5 & 51.8 \\                                                 
  Kimi-K2 & 38B & 6B& 69.5 & 65.7 & 76.5 & 69.2 & 73.5 \\                                        \bottomrule                     
  \end{tabular}                            
  \end{table} 
                                        
